Inference Networks for Sequential Monte Carlo in Graphical Models

We introduce a new approach for amortizing inference in directed graphical models by learning heuristic approximations to stochastic inverses, designed specifically for use as proposal distributions in sequential Monte Carlo methods. We describe a procedure for constructing and learning a structured neural network which represents an inverse factorization of the graphical model, resulting in a conditional density estimator that takes as input particular values of the observed random variables, and returns an approximation to the distribution of the latent variables. This recognition model can be learned offline, independent from any particular dataset, prior to performing inference. The output of these networks can be used as automatically-learned high-quality proposal distributions to accelerate sequential Monte Carlo across a diverse range of problem settings.

==> network-structure.tex <==
% !TEX root =  main.tex
%
%\begin{figure}
%\centering
%
%\begin{tikzpicture}
%
%  % Define nodes
%%  \node[obs](y){$t_n$};
%%  \node[obs,above=1.8em of y]  (x) {$z_{n}$}; %x_{nd}
%%  \node[latent, left=2.2em of x,yshift=0.5em] (w0) {${w_0}$};
%%  \node[latent, below=.6em of w0] (w1) {${w_1}$};
%%  \node[latent, below=.6em of w1] (w2) {${w_2}$};
%
%\node[obs](y1){$y_1$};
%\node[obs,right=1.5em of y1](y2){$y_2$};
%\node[latent,right=1.5em of y2](x1){$x_1$};
%\node[latent,right=1.5em of x1](x2){$x_2$};
%\node[latent,right=1.5em of x2](x3){$x_3$};
%
%\node[latent,above=2em of y1,xshift=-2em](h11){\color{black}{0}};
%\node[latent,right=1.5em of h11](h12){\color{black}{0}};
%\node[latent,right=1.5em of h12](h13){\color{black}{1}};
%\node[latent,right=1.5em of h13](h14){\color{black}{1}};
%\node[latent,right=1.5em of h14](h15){2};
%\node[latent,right=1.5em of h15](h16){2};
%
%\node[latent,above=2em of h11](h21){\color{black}{0}};
%\node[latent,right=1.5em of h21](h22){\color{black}{0}};
%\node[latent,right=1.5em of h22](h23){\color{black}{1}};
%\node[latent,right=1.5em of h23](h24){\color{black}{1}};
%\node[latent,right=1.5em of h24](h25){2};
%\node[latent,right=1.5em of h25](h26){2};
%
%  % Connect the nodes
%%  \edge {x,w0} {y} ; 
%%  \edge {x,w1} {y} ; 
%%  \edge {x,w2} {y} ; 
%    
%  % Plates
%%  \plate [inner xsep=1em,inner ysep=.4em,yshift=.2em]{xy} {(x)(y)} {\hbox{$N$\hspace{-.5em}}} ;
%%  \plate [inner xsep=.8em,inner ysep=.5em,yshift=.3em]{} {(w)(x)} {\hbox{$D$\hspace{-.5em}}} ;
%\end{tikzpicture}
%
%
%\caption{Neural network structure}
%\end{figure}
%


\begin{figure}
\centering

\begin{tikzpicture}

\node[obs](y1){$y_1$};
\node[obs,right=1.5em of y1](y2){$y_2$};
\node[latent,right=1.5em of y2](x1){$x_1$};
\node[latent,right=1.5em of x1](x2){$x_2$};
\node[latent,right=1.5em of x2](x3){$x_3$};

\node[latent,above=2em of y2,xshift=-6em](h11){\color{black}{0}};
\node[latent,right=1.5em of h11](h13){\color{black}{1}};
\node[latent,right=1.5em of h13](h15){\color{black}{2}};
\node[latent,right=1.5em of h15](h12){\color{black}{0}};
\node[latent,right=1.5em of h12](h14){\color{black}{1}};

\node[latent,above=2em of h11](h21){\color{black}{0}};
\node[latent,right=1.5em of h21](h23){\color{black}{1}};
\node[latent,right=1.5em of h23](h24){\color{black}{1}};
\node[latent,right=1.5em of h24](h22){\color{black}{0}};
\node[latent,right=1.5em of h22](h25){\color{black}{2}};

%\node[latent,above=2em of h23,xshift=1.5em,label={\hspace{-2.5em}$\tilde p(x_1|y_{1:2})$}](theta1){$\lambda_1$};
%\node[latent,right=1.5em of theta1,label={$\tilde p(x_2|x_1,y_{1:2})$}](theta2){$\lambda_2$};
%\node[latent,right=1.5em of theta2,label={\hspace{2.5em}$\tilde p(x_3|x_{1:2},y_{1:2})$}](theta3){$\lambda_3$};
\node[latent,above=2em of h23,xshift=1.5em,label={\hspace{-1em}$\tilde q(x_1|\lambda_1)$}](theta1){$\lambda_1$};
\node[latent,right=1.5em of theta1,label={$\tilde q(x_2|\lambda_2)$}](theta2){$\lambda_2$};
\node[latent,right=1.5em of theta2,label={\hspace{1em}$\tilde q(x_3|\lambda_3)$}](theta3){$\lambda_3$};

  % Connect the nodes
\edge[-,red]{y1}{h11,h12};
\edge[-,red]{y2}{h11,h12};
\edge[-,red]{h11,h12}{h21,h22};
\edge[-,red]{h21,h22}{theta1};

\edge[-,red]{y1}{h13,h14};
\edge[-,red]{y2}{h13,h14};
\edge[-,red]{h11,h12}{h23,h24};
\edge[-,red]{h21,h22}{theta2};

\edge[-,blue]{x1}{h13,h14};
\edge[-,blue]{h13,h14}{h23,h24};
\edge[-,blue]{h23,h24}{theta2};

\edge[-,green]{x2}{h15};
\edge[-,green]{h15}{h25};
\edge[-,green]{h25}{theta3};

\edge[-,red]{y1,y2}{h15};
\edge[-,red]{h11,h12}{h25};
\edge[-,red]{h21,h22}{theta3};

\edge[-,blue]{x1}{h15};
\edge[-,blue]{h13,h14}{h25};
\edge[-,blue]{h23,h24}{theta3};


  % Plates
%  \plate [inner xsep=1em,inner ysep=.4em,yshift=.2em]{xy} {(x)(y)} {\hbox{$N$\hspace{-.5em}}} ;
%  \plate [inner xsep=.8em,inner ysep=.5em,yshift=.3em]{} {(w)(x)} {\hbox{$D$\hspace{-.5em}}} ;
\end{tikzpicture}


\caption{Neural network structure}
\end{figure}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


